Playing for 3D Human Recovery

Image- and video-based 3D human recovery (i.e., pose and shape estimation) have achieved substantial progress. However, due to the prohibitive cost of motion capture, existing datasets are often limited in scale and diversity. In this work, we obtain massive human sequences by playing the video game with automatically annotated 3D ground truths. Specifically, we contribute GTA-Human, a large-scale 3D human dataset generated with the GTA-V game engine, featuring a highly diverse set of subjects, actions, and scenarios. More importantly, we study the use of game-playing data and obtain five major insights. First, game-playing data is surprisingly effective. A simple frame-based baseline trained on GTA-Human outperforms more sophisticated methods by a large margin. For video-based methods, GTA-Human is even on par with the in-domain training set. Second, we discover that synthetic data provides critical complements to the real data that is typically collected indoor. Our investigation into domain gap provides explanations for our data mixture strategies that are simple yet useful. Third, the scale of the dataset matters. The performance boost is closely related to the additional data available. A systematic study reveals the model sensitivity to data density from multiple key aspects. Fourth, the effectiveness of GTA-Human is also attributed to the rich collection of strong supervision labels (SMPL parameters), which are otherwise expensive to acquire in real datasets. Fifth, the benefits of synthetic data extend to larger models such as deeper convolutional neural networks (CNNs) and Transformers, for which a significant impact is also observed. We hope our work could pave the way for scaling up 3D human recovery to the real world. Homepage: https://caizhongang.github.io/projects/GTA-Human/

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> tables/3_benchmark.tex <==
\begin{table}[t!]
  \centering
  {
  \begin{tabular}{lrrrrrrcc}
    \toprule
     & 
    \multicolumn{2}{c}{Human3.6M \cite{ionescu2013human3}} & \multicolumn{2}{c}{MPI-INF-3DHP \cite{mehta2017monocular}} & 
    \multicolumn{2}{c}{3DPW \cite{von2018recovering}} & 
    \multicolumn{2}{c}{\name} \\
    
    \cmidrule(lr){2-3} 
    \cmidrule(lr){4-5} 
    \cmidrule(lr){6-7}
    \cmidrule(lr){8-9}
    
    Method &  
    MPJPE $\downarrow$ & PA $\downarrow$ & 
    MPJPE $\downarrow$ & PA $\downarrow$ & 
    MPJPE $\downarrow$ & PA $\downarrow$ &
    MPJPE $\downarrow$ & PA $\downarrow$ \\
    \midrule
    
    HMR \cite{kanazawa2018end}+ &
    77.9 & 55.8 & 107.2 & 74.1 & 98.5 & 61.7 & 186.8 & 94.7 \\
    
    SPIN \cite{kolotouros2019learning} &
    65.5 & 44.5 & 103.7 & 67.8 & 96.9 & 59.2 & 184.3 & 92.1 \\
    
    VIBE \cite{kocabas2020vibe} &
     65.9 & 41.5 & 97.7 & 63.4 & 93.5 & 56.5 & 166.6 & 89.5 \\
    \bottomrule
  \end{tabular}
  }
  \caption{\textbf{\name as a benchmark}. We directly evaluate state-of-the-art (SOTA) methods on \name without finetuning and compare the results with other standard benchmarks. 
%   \name has two ideal traits as a benchmark: it is 1) \emph{challenging}: methods that perform well on other benchmarks give larger errors on \name; 2) \emph{indicative}: methods that perform relatively well \name also perform relatively well other benchmarks. 
  Since methods are not trained on 3DPW but still achieve good results, this may indicate that there exists domain gaps between real and synthetic data.
  PA: PA-MPJPE. +: our strong baseline of HMR.}
  \label{tab:benchmark}
\end{table}

==> tables/9_characters.tex <==
\begin{table}[t!]
  \caption{A manual investigation into character appearances. M: male; F: female. }
  \label{tab:characters}
  \centering
  \begin{tabular}{lrrrrr}
    \toprule
    Clothing & M & F & White & Black & Asian \\
    \midrule
    Formal      & 11\% & 9\% & 14\% & 5\% & 1\% \\
    Semi-formal & 33\% & 11\% & 18\% & 18\%	& 8\% \\
    Casual      & 25\% & 11\% & 18\% & 16\% & 2\% \\
    \bottomrule
  \end{tabular}
\end{table}


==> tables/9_more_comparison.tex <==
% \begin{table}
%   \caption{SOTA and their results on 3DPW test}
%   \label{tab:supp_sotas}
%   \centering
%   \begin{tabular}{p{0.5\linewidth}|c|c|c}
%     \toprule
%      Title & Venue & MPJPE & PA-MPJPE \\
%      \midrule
%      % TOG 2020
%      XNect: Real-time Multi-Person 3D Motion Capture with a Single RGB Camera & TOG 2020 & 103.3 & 60.7 \\
%     \midrule
%     % ECCV 2020
%      Towards Part-aware Monocular 3D Human Pose Estimation: An Architecture Search Approach & ECCV 2020 & - & - \\
%      \midrule
%      Beyond Weak Perspective for Monocular 3D Human Pose Estimation & ECCV 2020 & 83.154 & 59.703 \\
%      \midrule
%      Hierarchical Kinematic Human Mesh Recovery & ECCV 2020 & - & - \\
%      \midrule
%     I2L-MeshNet: Image-to-Lixel Prediction
%     Network for Accurate 3D Human Pose and Mesh Estimation from a Single RGB Image & ECCV 2020 & 93.2 & 58.6 \\
%     \midrule
%     HMOR: Hierarchical Multi-Person Ordinal Relations for Monocular Multi-Person 3D Pose Estimation & ECCV 2020 & 87.7 & 57.4 \\
%     \midrule
%     Pose2Mesh: Graph Convolutional Network for 3D Human Pose and Mesh Recovery from a 2D Human Pose & ECCV 2020 & 89.2 & 58.9 \\
%     \midrule
%     % CVPR 2021
%     AGORA: Avatars in Geography Optimized for Regression Analysis & CVPR 2021 & 85.7 & 55.3 \\
%     \midrule
%     Beyond Static Features for
%     Temporally Consistent 3D Human Pose and Shape from a Video & CVPR 2021 & 95.0 & 55.8 \\
%     \midrule
%     Bilevel Online Adaptation for Out-of-Domain Human Mesh Reconstruction & CVPR 2021 & 77.2 & 49.5 \\
%     \midrule
%      HybrIK: A Hybrid Analytical-Neural Inverse Kinematics Solution for 3D Human Pose and Shape Estimation & CVPR 2021 & 80.0 & 48.8 \\
%     \midrule
%     End-to-End Human Pose and Mesh Reconstruction with Transformers & CVPR 2021 & 77.1 & 47.9 \\ 
%     \midrule
%     % arXiv
%      Exemplar Fine-Tuning for 3D Human Model Fitting Towards In-the-Wild 3D Human Pose Estimation & arXiv & - & 52.2 \\
%      \midrule
%       Human Mesh Recovery from Multiple Shots & arXiv & - & 57.8 \\
%      \midrule
%          Human Body Model Fitting by Learned Gradient Descent & arXiv & - & 55.9 \\
%     \midrule
%         CenterHMR: Multi-Person Center-based Human Mesh Recovery & arXiv & 76.0 & 46.7 \\
%     \midrule
%     \bottomrule
%   \end{tabular}
% \end{table}


\begin{table*}[t]
  \centering
  \caption{\textbf{More results on the unreasonable effectiveness of data.} \name enables a relatively simple HMR baseline to outperform a series of newer works, some of which even employs more sophisticated strategies such as an optimization step (Opt) or temporal information (Video). In addition, \name also improves PARE, a SOTA method, by a considerable margin. Evaluation is conducted on 3DPW \cite{von2018recovering} test set, without using any 3DPW data in the train set}
  \label{tab:more_on_effectiveness}
  \vspace{2mm}
  \begin{tabular}{lccccrrrr}
    \hline
    Method & Year & Mixture & Regis. & Video & MPJPE $\downarrow$ & PA-MPJPE $\downarrow$ \\
    \hline
    SMPLify \cite{bogo2016keep}
    & 2016 & - & \cm &  -  & -  & 106.1 \\ % cite from song2020human
    
    HMR \cite{kanazawa2018end}          
    & 2018 & - & -  &  -  &  130.0  & 76.7 \\
    
    Kanazawa \etal \cite{kanazawa2019learning}
    & 2019 & - & -  & \cm &  116.5  & 72.6 \\

    GraphCMR \cite{kolotouros2019convolutional} 
    & 2019 & - & -  &  -  &  -      & 70.2 \\

    DSD+SATN \cite{sun2019human}
    & 2019 & - & -  & \cm & - & 69.5 \\

    SPIN \cite{kolotouros2019learning}  
    & 2019 & - & \cm &  -  &   96.9  & 59.2 \\
    
    I2L-MeshNet \cite{moon2020i2l}
    & 2020 & - & -  & \cm &  93.2  & 58.6 \\
    
    Pavlakos \etal \cite{pavlakos2020human}
    & 2020 & - & -  & \cm &  -  & 57.8 \\
    
    VIBE \cite{kocabas2020vibe}         
    & 2020 & - & -  & \cm &  93.5  & 56.5 \\

    Song \etal \cite{song2020human}
    & 2020 & - & \cm &  -  &  -  & 55.9 \\
    
    TCMR \cite{choi2021beyond}
    & 2021 & - & -  & \cm & 95.0 & 55.8 \\
    
    ROMP \cite{sun2020monocular}
    & 2021 & - & -  & - & 91.3 & 54.9 \\
    
    PARE \cite{kocabas2021pare}
    & 2021 & - & -  & -  & 82.0 & 50.9 \\
    
    HybrIK \cite{li2020hybrik}
    & 2021 & - & - & - & 80.0 & 48.8 \\
    
    \hline
    HMR                             
    & 2022 & BT & -  &  -  &  88.7  & 56.0 \\
    HMR                             
    & 2022 & FT & -  &  -  &  91.4  & 55.5 \\
    SPIN                             
    & 2022 & FT & -  & -  & 83.1 & 52.0 \\
    PARE
    & 2022 & FT & -  & -  & 77.6 & 48.6 \\
    \hline
  \end{tabular}
\end{table*}

==> tables/rebuttal_more_baselines.tex <==
\begin{table}[h]
  \centering
  \vspace{-2mm}
  \begin{tabular}{lccc}
    \toprule
    Method & MPJPE  & PA-MPJPE & PVE  \\
    \midrule
     PARE & 82.0 & 50.9 & 97.9 \\
     PARE(FT) & 77.6\textcolor{ao}{(-4.4)} & 48.6\textcolor{ao}{(-2.3)} & 92.3\textcolor{ao}{(-5.6)}\\
    % \midrule
    %  HybrIK &  \\
    %  HybrIK(FT) &  \\
    \bottomrule
  \end{tabular}
  \vspace{-2mm}
  \caption{PARE with GTA-Human on 3DPW test set.}
  \label{tab:rebuttal_more_baselines}
  \vspace{-2mm}
\end{table}

==> tables/rebuttal_more_benchmarks.tex <==
\begin{table}[h]
  \centering
  \vspace{-2mm}
  \begin{tabular}{lcccc}
    \toprule
    & \multicolumn{2}{c}{Human3.6M} & \multicolumn{2}{c}{MI3} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5}
    Method & 
    MPJPE  & PA & 
    MPJPE  & PA  \\
    \midrule
    %  VIBE & 65.9    & 41.5 & 97.7 & 63.4 \\
    %  I2L & 55.7 & 41.7 & - & - \\
    %  SPIN   & -    & 41.1 & 105.2 & 67.5 \\
     SPIN*      & 62.4 & 41.9 & 103.7 & 67.9 \\
     SPIN(FT)   & 60.9 & 40.8 & 96.4 & 67.0 \\
     $\Delta$ & \textcolor{ao}{(-1.5)} & \textcolor{ao}{(-1.1)} & \textcolor{ao}{(-7.3)} & \textcolor{ao}{(-0.9)} \\
    \bottomrule
  \end{tabular}
  \vspace{-2mm}
  \caption{More experiments on Human3.6M and MPI-INF-3DHP. *: official pretrained model provided by SPIN authors. }
  \label{tab:rebuttal_more_benchmarks}
  \vspace{-2mm}
\end{table}
